Weakly-Supervised Learning of Visual Relations in Multimodal Pretraining

Recent work in vision-and-language pretraining has investigated supervised signals from object detection data to learn better, fine-grained multimodal representations. In this work, we take a step further and explore how we can tap into supervision from small-scale visual relation data. In particular, we propose two pretraining approaches to contextualise visual entities in a multimodal setup. With verbalised scene graphs, we transform visual relation triplets into structured captions, and treat them as additional image descriptions. With masked relation prediction, we further encourage relating entities from image regions with visually masked contexts. When applied to strong baselines pretrained on large amounts of Web data, zero-shot evaluations on both coarse-grained and fine-grained tasks show the efficacy of our methods in learning multimodal representations from weakly-supervised relations data.

==> tables/2023-03-09_14m_fixed.tex <==
\begin{tabular}{lrllllllll}
\toprule
{} &  {} &  {}                                   &       Flickr30k  &       Flickr30k  &       MS-COCO  &       MS-COCO  &      VALSE  &    VSR Dev/Test  &       SVO-Probes \\
{} &  {} &                                 model &           TR@1/5 &           IR@1/5 &         TR@1/5 &         IR@1/5 &      Acc\_r &              Acc &           Acc\_r \\
\midrule
0  &      0 &                         albef-14m@200k &      83.2 / 95.1 &      66.1 / 88.2 &    66.4 / 87.9 &    49.6 / 76.3 &        70.8 &      63.2 / 61.3 &             87.8 \\
% 16 &      0 &                         albef-14m@500k &      82.2 / 95.5 &      66.1 / 85.8 &    64.8 / 86.6 &    49.1 / 74.6 &        72.2 &      60.4 / 59.4 &             86.7 \\
1  &      1 &                    albef-viz4-14m@200k &      78.5 / 95.1 &      64.0 / 86.9 &    64.2 / 86.8 &    48.9 / 76.0 &        71.1 &      63.3 / 58.7 &             87.7 \\
% 17 &      1 &                    albef-viz4-14m@500k &      78.7 / 94.3 &      64.3 / 86.0 &    64.2 / 86.7 &    48.5 / 75.2 &        71.0 &      62.6 / 59.6 &             87.8 \\
% 2  &      2 &                     albef-vsg-14m@200k &      79.3 / 94.9 &      61.8 / 85.0 &    62.6 / 85.9 &    46.9 / 74.8 &        69.9 &      63.9 / 61.7 &             86.7 \\
18 &      2 &                     albef-vsg-14m@500k &      78.3 / 94.3 &      62.8 / 85.4 &    64.2 / 86.2 &    48.0 / 74.7 &        70.7 &      63.3 / 61.3 &             87.9 \\
% 3  &      3 &                  albef-relclf-14m@200k &      80.3 / 94.1 &      65.4 / 87.0 &    67.4 / 88.4 &    50.0 / 77.2 &        72.3 &      62.6 / 59.4 &             87.6 \\
19 &      3 &                  albef-relclf-14m@500k &      81.9 / 95.0 &      66.6 / 86.7 &    68.2 / 88.8 &    50.5 / 76.8 &        71.2 &      62.0 / 60.7 &             87.4 \\
% 4  &      4 &     albef-mix-models-viz4-vsg-14m@200k &      75.4 / 92.8 &      60.0 / 84.3 &    59.3 / 84.3 &    44.8 / 73.5 &        72.0 &      61.8 / 56.8 &             86.5 \\
% 20 &      4 &     albef-mix-models-viz4-vsg-14m@500k &      79.1 / 94.8 &      65.2 / 86.9 &    63.4 / 87.1 &    48.5 / 75.7 &        71.2 &      63.2 / 59.2 &             87.8 \\
21 &      5 &  albef-mix-models-viz4-relclf-14m@500k &      83.0 / 95.5 &      67.4 / 88.1 &    67.9 / 89.3 &    51.1 / 77.8 &        70.7 &      63.2 / 60.8 &             87.6 \\
% 5  &      5 &  albef-mix-models-viz4-relclf-14m@200k &      79.7 / 93.8 &      62.3 / 85.6 &    64.7 / 87.9 &    47.8 / 76.2 &        71.9 &      62.4 / 59.7 &             87.3 \\
22 &      6 &   albef-mix-models-relclf-vsg-14m@500k &      80.3 / 93.7 &      65.1 / 86.0 &    66.3 / 87.8 &    49.1 / 76.1 &        70.4 &      64.6 / 61.3 &             87.5 \\
% 6  &      6 &   albef-mix-models-relclf-vsg-14m@200k &      75.2 / 91.9 &      61.7 / 84.6 &    62.8 / 86.1 &    46.7 / 74.8 &        71.0 &      61.7 / 59.5 &             86.4 \\
23 &      7 &          albef-mix-models-all-14m@500k &      79.0 / 94.3 &      63.5 / 86.5 &    65.5 / 88.3 &    49.3 / 76.8 &        69.6 &      62.3 / 60.3 &             87.6 \\
% 7  &      7 &          albef-mix-models-all-14m@200k &      70.5 / 91.0 &      57.6 / 81.6 &    59.1 / 84.4 &    44.1 / 73.0 &        67.9 &      61.1 / 58.3 &             86.2 \\
\midrule
% 24 &      8 &                     xvlm-500k-14m@500k &      82.1 / 94.9 &      65.0 / 85.9 &    64.7 / 86.5 &    49.0 / 74.6 &        71.3 &      61.1 / 60.5 &             87.3 \\
8  &      8 &                     xvlm-500k-14m@200k &      84.2 / 96.6 &      68.0 / 87.8 &    67.3 / 88.4 &    50.7 / 76.9 &        72.2 &      64.5 / 62.5 &             87.7 \\
25 &      9 &                     xvlm-viz4-14m@500k &      81.4 / 95.4 &      64.5 / 86.5 &    65.6 / 86.9 &    48.9 / 75.6 &        69.2 &      65.2 / 60.7 &             87.6 \\
% 9  &      9 &                     xvlm-viz4-14m@200k &      80.3 / 94.4 &      62.1 / 86.5 &    64.1 / 87.0 &    47.5 / 75.6 &        69.2 &      62.6 / 61.4 &             87.6 \\
% 11 &     11 &                   xvlm-relclf-14m@200k &      80.3 / 94.9 &      64.4 / 87.6 &    67.6 / 89.8 &    50.7 / 78.6 &        70.6 &      64.5 / 60.5 &             87.5 \\
26 &     10 &                   xvlm-relclf-14m@500k &      83.7 / 96.4 &      66.6 / 88.3 &    68.3 / 89.1 &    52.1 / 78.0 &        71.2 &      65.0 / 62.5 &             88.3 \\
10 &     10 &                      xvlm-vsg-14m@200k &      81.0 / 94.7 &      66.1 / 87.8 &    65.8 / 87.9 &    49.4 / 76.4 &        71.1 &      63.8 / 62.6 &             87.8 \\

27 &     11 &      xvlm-mix-models-viz4-vsg-14m@500k &      81.9 / 95.2 &      66.0 / 87.7 &    66.0 / 87.9 &    49.5 / 76.2 &        70.0 &      66.8 / 63.1 &             87.6 \\
% 12 &     12 &      xvlm-mix-models-viz4-vsg-14m@200k &      80.6 / 95.1 &      64.3 / 86.6 &    65.4 / 87.9 &    48.8 / 76.4 &        70.2 &      64.4 / 61.2 &             87.7 \\
% 13 &     13 &   xvlm-mix-models-viz4-relclf-14m@200k &      79.8 / 94.6 &      61.9 / 85.8 &    65.6 / 88.2 &    48.7 / 77.0 &        71.4 &      64.2 / 60.6 &             87.2 \\
28 &     12 &   xvlm-mix-models-viz4-relclf-14m@500k &      81.3 / 95.2 &      65.3 / 87.2 &    67.2 / 88.4 &    50.4 / 77.0 &        71.0 &      64.8 / 61.1 &             87.9 \\
29 &     13 &    xvlm-mix-models-relclf-vsg-14m@500k &      80.2 / 95.8 &      66.4 / 87.0 &    67.4 / 88.3 &    50.1 / 77.0 &        73.3 &      68.4 / 63.5 &             88.1 \\
% 14 &     14 &    xvlm-mix-models-relclf-vsg-14m@200k &      78.8 / 94.2 &      63.0 / 86.3 &    64.8 / 87.9 &    48.5 / 76.8 &        72.2 &      65.2 / 62.1 &             87.3 \\
% 15 &     15 &           xvlm-mix-models-all-14m@200k &      79.6 / 94.8 &      61.2 / 85.0 &    63.7 / 87.2 &    47.7 / 75.5 &        71.3 &      63.7 / 60.9 &             87.1 \\
30 &     14 &           xvlm-mix-models-all-14m@500k &      79.6 / 95.4 &      63.7 / 86.0 &    65.9 / 87.9 &    49.3 / 76.9 &        70.8 &      64.8 / 60.9 &             87.9 \\
\bottomrule
\end{tabular}

==> tables/2023-03-09_14m_minicoco.tex <==
\begin{tabular}{lrllllllll}
\toprule
{} &  {} &  {}                          &       Flickr30k  &       Flickr30k  &       MS-COCO  &       MS-COCO  &      VALSE  &    VSR Dev/Test  &       SVO-Probes \\
{} &  {} &                        model &           TR@1/5 &           IR@1/5 &         TR@1/5 &         IR@1/5 &      Acc\_r &              Acc &           Acc\_r \\
\midrule
43  &&                         albef-14m &      81.4 / 95.5 &      65.5 / 86.8 &    66.5 / 87.4 &    49.1 / 76.4 &        71.8 &      63.4 / 60.7 &             86.9 \\
% 362 &&                    albef-viz4-14m &      82.0 / 94.9 &      65.5 / 86.6 &    66.9 / 88.0 &    49.5 / 76.3 &        71.3 &      62.9 / 59.7 &             88.0 \\
118 &&                     albef-vsg-14m &      76.8 / 94.1 &      63.5 / 85.0 &    63.3 / 86.6 &    47.1 / 74.7 &        71.6 &      64.4 / 62.4 &             87.1 \\
332 &&                  albef-relclf-14m &      82.8 / 95.2 &      66.0 / 87.0 &    68.1 / 89.4 &    50.9 / 77.6 &        71.8 &      62.5 / 61.8 &             88.2 \\
% 269 &&     albef-mix-models-viz4-vsg-14m &      79.2 / 94.7 &      64.6 / 86.6 &    64.1 / 87.2 &    48.7 / 76.0 &        71.1 &      64.4 / 59.3 &             87.5 \\
% 203 &&  albef-mix-models-viz4-relclf-14m &      80.1 / 94.8 &      64.2 / 86.4 &    66.0 / 88.0 &    49.3 / 76.9 &        71.2 &      62.2 / 58.6 &             86.9 \\
244 &&   albef-mix-models-relclf-vsg-14m &      79.2 / 94.3 &      64.9 / 86.0 &    66.3 / 88.5 &    49.2 / 76.3 &        71.5 &      64.9 / 61.8 &             87.4 \\
% 191 &&          albef-mix-models-all-14m &      79.7 / 94.7 &      63.6 / 86.0 &    65.0 / 87.7 &    49.0 / 76.5 &        69.4 &      62.5 / 59.2 &             87.5 \\
\midrule
305 &&                    xvlm-500k-14m &      83.6 / 96.2 &      67.0 / 87.4 &    67.1 / 87.6 &    50.7 / 76.4 &        72.2 &      63.2 / 61.9 &             88.2 \\
% 65  &&                    xvlm-viz4-14m &      80.7 / 94.6 &      65.1 / 87.2 &    65.3 / 87.1 &    48.5 / 76.2 &        70.0 &      63.4 / 60.3 &             88.2 \\
91  &&                     xvlm-vsg-14m &      81.7 / 96.4 &      66.3 / 87.9 &    66.8 / 87.5 &    49.6 / 76.1 &        69.5 &      63.6 / 61.7 &             88.0 \\
495 &&                  xvlm-relclf-14m &      82.4 / 96.1 &      67.5 / 88.5 &    68.8 / 90.0 &    52.1 / 78.6 &        71.9 &      64.5 / 63.4 &             88.1 \\
% 287 &&     xvlm-mix-models-viz4-vsg-14m &      81.1 / 95.7 &      65.7 / 87.6 &    66.4 / 87.8 &    49.8 / 76.8 &        70.8 &      65.7 / 63.5 &             88.1 \\
% 58  &&  xvlm-mix-models-viz4-relclf-14m &      82.9 / 96.6 &      66.2 / 88.1 &    67.9 / 89.5 &    50.8 / 77.5 &        71.1 &      64.5 / 60.7 &             87.7 \\
262 &&   xvlm-mix-models-relclf-vsg-14m &      81.4 / 95.3 &      65.5 / 87.0 &    67.0 / 88.9 &    49.9 / 77.1 &        71.9 &      67.1 / 62.9 &             87.8 \\
% 276 &&          xvlm-mix-models-all-14m &      81.4 / 95.8 &      64.2 / 86.3 &    66.6 / 88.3 &    49.4 / 77.0 &        71.6 &      64.5 / 61.5 &             87.8 \\
\bottomrule
\end{tabular}

==> tables/2023-03-09_4m_minicoco.tex <==
\begin{tabular}{lrllllllll}
\toprule
{} &  {} &  {}                      &       Flickr30k  &       Flickr30k  &       MS-COCO  &       MS-COCO  &      VALSE  &    VSR Dev/Test  &       SVO-Probes \\
{} &  {} &                    model &           TR@1/5 &           IR@1/5 &         TR@1/5 &         IR@1/5 &      Acc\_r &              Acc &           Acc\_r \\
\midrule
10  &&                    albef-500k &      76.8 / 92.8 &      60.5 / 84.1 &    62.3 / 86.8 &    46.4 / 74.5 &        68.5 &      61.9 / 59.8 &             86.7 \\
% 318 &&                    albef-viz4 &      78.3 / 93.9 &      62.7 / 85.4 &    63.7 / 85.9 &    48.4 / 75.4 &        69.7 &      61.4 / 59.5 &             86.9 \\
466 &&                     albef-vsg &      74.9 / 91.8 &      59.8 / 82.7 &    61.6 / 85.6 &    46.0 / 73.5 &        68.2 &      64.1 / 60.4 &             86.7 \\
184 &&                  albef-relclf &      76.9 / 93.2 &      61.1 / 84.1 &    64.4 / 86.6 &    48.2 / 75.4 &        70.0 &      60.7 / 60.9 &             86.9 \\
% 15  &&     albef-mix-models-viz4-vsg &      75.0 / 91.6 &      60.1 / 83.2 &    61.6 / 86.5 &    47.0 / 74.8 &        70.6 &      61.9 / 59.3 &             86.6 \\
% 486 &&  albef-mix-models-viz4-relclf &      76.7 / 91.3 &      61.2 / 84.2 &    64.6 / 87.3 &    48.5 / 75.9 &        69.5 &      63.3 / 59.9 &             86.6 \\
244 &&   albef-mix-models-relclf-vsg &      75.9 / 93.1 &      60.0 / 83.0 &    63.2 / 86.6 &    46.4 / 74.5 &        70.7 &      63.5 / 60.6 &             86.1 \\
% 232 &&          albef-mix-models-all &      78.2 / 93.2 &      61.3 / 83.5 &    64.7 / 87.5 &    49.0 / 76.0 &        70.6 &      62.8 / 59.3 &             86.4 \\
\midrule
140 &&                    xvlm-500k &      79.3 / 95.1 &      63.4 / 85.8 &    66.0 / 88.3 &    49.2 / 76.0 &        69.8 &      65.1 / 62.5 &             87.2 \\
% 352 &&                    xvlm-viz4 &      77.8 / 94.1 &      61.0 / 84.8 &    64.4 / 87.6 &    48.3 / 75.9 &        70.3 &      62.7 / 60.9 &             86.8 \\
23  &&                     xvlm-vsg &      77.0 / 93.1 &      61.9 / 84.2 &    63.3 / 86.4 &    47.3 / 74.7 &        69.1 &      63.7 / 61.8 &             87.3 \\
159 &&                  xvlm-relclf &      79.7 / 95.1 &      63.0 / 85.6 &    66.6 / 88.5 &    50.1 / 77.2 &        70.6 &      63.8 / 60.8 &             86.9 \\
% 411 &&     xvlm-mix-models-viz4-vsg &      78.5 / 93.4 &      62.4 / 85.4 &    64.5 / 86.6 &    48.2 / 75.2 &        68.8 &      67.0 / 63.5 &             87.2 \\
% 84  &&  xvlm-mix-models-viz4-relclf &      79.3 / 95.4 &      62.5 / 85.2 &    65.6 / 87.8 &    48.3 / 76.2 &        70.7 &      62.7 / 60.6 &             86.5 \\
302 &&   xvlm-mix-models-relclf-vsg &      78.4 / 93.3 &      62.3 / 85.6 &    65.9 / 87.9 &    49.2 / 76.0 &        71.1 &      65.5 / 62.0 &             86.9 \\
% 385 &&          xvlm-mix-models-all &      77.1 / 92.7 &      61.4 / 84.0 &    64.6 / 87.4 &    48.2 / 75.9 &        72.1 &      66.1 / 63.3 &             87.1 \\
\bottomrule
\end{tabular}

==> tables/2023-03-10_14m_minicocoIR.tex <==
\begin{tabular}{lrllllllll}
\toprule
{} &  {} &  {}                      &       Flickr30k  &       Flickr30k  &       MS-COCO  &       MS-COCO  &      VALSE  &    VSR Dev/Test  &       SVO-Probes \\
{} &  {} &                    model &           TR@1/5 &           IR@1/5 &         TR@1/5 &         IR@1/5 &      Acc\_r &              Acc &           Acc\_r \\
\midrule
10  &&                    albef-500k &      76.8 / 92.8 &      60.5 / 84.1 &    62.3 / 86.8 &    46.4 / 74.5 &        68.5 &      61.9 / 59.8 &             86.7 \\
466 &&                     albef-vsg &      74.9 / 91.8 &      59.8 / 82.7 &    61.6 / 85.6 &    46.0 / 73.5 &        68.2 &      64.1 / 60.4 &             86.7 \\
184 &&                  albef-relclf &      76.9 / 93.2 &      61.1 / 84.1 &    64.4 / 86.6 &    48.2 / 75.4 &        70.0 &      60.7 / 60.9 &             86.9 \\
244 &&   albef-mix-models-relclf-vsg &      75.9 / 93.1 &      60.0 / 83.0 &    63.2 / 86.6 &    46.4 / 74.5 &        70.7 &      63.5 / 60.6 &             86.1 \\
\midrule
140 &&                    xvlm-500k &      79.3 / 95.1 &      63.4 / 85.8 &    66.0 / 88.3 &    49.2 / 76.0 &        69.8 &      65.1 / 62.5 &             87.2 \\
23  &&                     xvlm-vsg &      77.0 / 93.1 &      61.9 / 84.2 &    63.3 / 86.4 &    47.3 / 74.7 &        69.1 &      63.7 / 61.8 &             87.3 \\
159 &&                  xvlm-relclf &      79.7 / 95.1 &      63.0 / 85.6 &    66.6 / 88.5 &    50.1 / 77.2 &        70.6 &      63.8 / 60.8 &             86.9 \\
302 &&   xvlm-mix-models-relclf-vsg &      78.4 / 93.3 &      62.3 / 85.6 &    65.9 / 87.9 &    49.2 / 76.0 &        71.1 &      65.5 / 62.0 &             86.9 \\
\bottomrule
\end{tabular}

% albef-14m     	    150000	83.1 / 95.7	66.1 / 88.1	66.6 / 88.5	49.3 / 76.4	71.3	63.6 / 60.3	87.4
% albef-vsg-14m	        300000	80.9 / 96.2	63.4 / 86.0	64.1 / 86.5	48.3 / 75.2	71.3	63.2 / 61.5	87.2
% albef-relclf-14m  	200000	80.3 / 94.1	65.4 / 87.0	67.4 / 88.4	50.0 / 77.2	72.3	62.6 / 59.3	87.6
% albef-relclf-vsg-14m	350000	78.6 / 94.5	64.2 / 85.6	65.1 / 87.6	48.7 / 76.2	71.8	63.7 / 61.9	87.7

% xvlm-500k-14m	        200000	84.2 / 96.6	68.0 / 87.8	67.3 / 88.4	50.7 / 76.9	72.2	64.5 / 62.5	87.7
% xvlm-vsg-14m	        200000	81.0 / 94.7	66.1 / 87.8	65.8 / 87.9	49.4 / 76.4	71.1	64.0 / 62.7	87.8
% xvlm-relclf-14m	    350000	82.9 / 95.4	68.1 / 88.7	68.8 / 90.0	52.4 / 78.5	70.0	65.0 / 62.4	88.1
% xvlm-relclf-vsg-14m	250000	81.2 / 93.9	64.6 / 87.3	67.3 / 88.1	50.2 / 77.6	71.7	66.3 / 61.7	87.8

==> tables/2023-03-10_4m_minicocoIR.tex <==
\begin{tabular}{lrllllllll}
\toprule
{} &  {} &  {}                      &       Flickr30k  &       Flickr30k  &       MS-COCO  &       MS-COCO  &      VALSE  &    VSR Dev/Test  &       SVO-Probes \\
{} &  {} &                    model &           TR@1/5 &           IR@1/5 &         TR@1/5 &         IR@1/5 &      Acc\_r &              Acc &           Acc\_r \\
\midrule
10  &&                    albef-500k &      76.8 / 92.8 &      60.5 / 84.1 &    62.3 / 86.8 &    46.4 / 74.5 &        68.5 &      61.9 / 59.8 &             86.7 \\
466 &&                     albef-vsg &      74.9 / 91.8 &      59.8 / 82.7 &    61.6 / 85.6 &    46.0 / 73.5 &        68.2 &      64.1 / 60.4 &             86.7 \\
184 &&                  albef-relclf &      76.9 / 93.2 &      61.1 / 84.1 &    64.4 / 86.6 &    48.2 / 75.4 &        70.0 &      60.7 / 60.9 &             86.9 \\
244 &&   albef-mix-models-relclf-vsg &      75.9 / 93.1 &      60.0 / 83.0 &    63.2 / 86.6 &    46.4 / 74.5 &        70.7 &      63.5 / 60.6 &             86.1 \\
\midrule
140 &&                    xvlm-500k &      79.3 / 95.1 &      63.4 / 85.8 &    66.0 / 88.3 &    49.2 / 76.0 &        69.8 &      65.1 / 62.5 &             87.2 \\
23  &&                     xvlm-vsg &      77.0 / 93.1 &      61.9 / 84.2 &    63.3 / 86.4 &    47.3 / 74.7 &        69.1 &      63.7 / 61.8 &             87.3 \\
159 &&                  xvlm-relclf &      79.7 / 95.1 &      63.0 / 85.6 &    66.6 / 88.5 &    50.1 / 77.2 &        70.6 &      63.8 / 60.8 &             86.9 \\
302 &&   xvlm-mix-models-relclf-vsg &      78.4 / 93.3 &      62.3 / 85.6 &    65.9 / 87.9 &    49.2 / 76.0 &        71.1 &      65.5 / 62.0 &             86.9 \\
\bottomrule
\end{tabular}

% albef-500k        100000  78.4 / 93.5	61.2 / 84.6	63.9 / 86.5	47.4 / 74.9	68.9	61.4 / 60.3	87.4
% albef-vsg	        250000	74.9 / 92.1	59.6 / 82.3	62.8 / 85.6	46.0 / 73.6	68.9	62.7 / 61.7	86.6
% albef-relclf  	250000	76.9 / 93.2	61.1 / 84.1	64.4 / 86.6	48.2 / 75.4	70.0	60.7 / 60.9	86.9
% albef-relclf-vsg	400000	76.8 / 92.9	61.1 / 83.3	64.0 / 86.9	47.6 / 75.1	70.1	64.3 / 60.7	86.2

% xvlm-500k	        100000	80.4 / 94.8	63.7 / 86.4	66.4 / 87.8	49.1 / 76.3	68.5	64.0 / 61.7	87.0
% xvlm-vsg	        200000	75.4 / 93.0	61.3 / 84.2	62.8 / 85.9	46.7 / 74.2	67.9	64.3 / 62.7	87.2
% xvlm-relclf	    250000	80.0 / 95.3	63.7 / 85.4	65.6 / 88.7	50.0 / 76.8	70.4	64.1 / 62.4	87.0
% xvlm-relclf-vsg	450000	78.9 / 93.2	61.5 / 84.6	65.1 / 87.1	48.8 / 75.4	70.1	65.3 / 62.5	87.5

==> tables/2023-03-15_best_overall_test.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{ll|cccc|ccc}
\toprule
{} &             {} &          \multicolumn{2}{c}{\textbf{Flickr30k}}  &     \multicolumn{2}{c|}{\textbf{MS-COCO}} &           \textbf{VALSE}  &    \textbf{VSR}  &           \textbf{SVO-Probes} \\
\textbf{Model} &          \textbf{Checkpoint}  &       TR@1/5  &          IR@1/5  &        TR@1/5 &         IR@1/5 &             Acc$_\text{r}$ &    Dev / Test Acc &                     Acc$_\text{r}$ \\
\midrule
\gray{CLIPs} & \citet{clip} & \gray{88.0 / ?} & \gray{68.7 / ?} & \gray{58.4 / ?} & \gray{37.8 / ?} & \gray{64.0} & \gray{? / ?} & \gray{81.6} \\
\midrule
% \gray{ALBEF$_\text{4M}$} & \citet{clip} & \gray{85.2 / ?} & \gray{69.4 / ?} & \gray{69.7 / ?} & \gray{51.1 / ?} & \gray{69.1} & \gray{? / 57.3} & \gray{87.6} \\
\albefb &       200{,}000 &      77.9 / 92.7 &      61.3 / 83.6 &    63.6 / 86.1 &    47.4 / 74.5 &        69.4 &      63.7 / 60.1 &             86.6 \\
\realbefb &     350{,}000 &      76.5 / 93.0 &      61.7 / 84.0 &    63.9 / 86.7 &    47.3 / 74.8 &        70.8 &      65.5 / 60.2 &             86.7 \\
% \gray{X-VLM$_\text{4M}$} & \citet{clip} & \gray{85.3 / ?} & \gray{71.9 / ?} & \gray{70.8 / ?} & \gray{55.6 / ?} & \gray{72.4} & \gray{? / 63.0} & \gray{88.9} \\
\xvlmb &        100{,}000 &      \textbf{80.4} / \textbf{94.8} &      \textbf{63.7} / \textbf{86.4} &    66.4 / 87.8 &    49.1 / \textbf{76.3} &        68.5 &      64.0 / 61.7 &             87.0 \\
\rexvlmb &     250{,}000 &      77.6 / 94.4 &      61.8 / 84.3 &    \textbf{66.8} / \textbf{88.2} &    \textbf{49.4} / \textbf{76.3} &        \textbf{71.2} &      \textbf{66.6} / \textbf{62.6} &             \textbf{87.2} \\
\midrule
% \gray{ALBEF$_\text{14M}$} & \citet{clip} & \gray{90.9 / ?} & \gray{75.9 / ?} & \gray{73.2 / ?} & \gray{54.8 / ?} & \gray{69.4} & \gray{? / 58.3} & \gray{88.6} \\
\albefl &      250{,}000 &      \textbf{84.1} / 94.6 &      67.3 / 87.6 &    66.8 / 87.9 &    49.7 / 76.5 &        71.4 &      62.4 / 61.3 &             87.5 \\
\realbefl &    500{,}000 &      80.3 / 93.7 &      65.1 / 86.0 &    66.3 / 87.8 &    49.1 / 76.1 &        70.4 &      64.6 / 61.3 &             87.7 \\
% \gray{X-VLM$_\text{16M}$} & \citet{clip} & \gray{87.7 / ?} & \gray{74.9 / ?} & \gray{71.6 / ?} & \gray{56.1 / ?} & \gray{74.5} & \gray{? / 64.3} & \gray{90.0} \\
\xvlml &       150{,}000 &      83.5 / 95.5 &      \textbf{67.5} / \textbf{88.6} &    \textbf{67.6} / 87.9 &    \textbf{50.6} / \textbf{77.1} &        70.9 &      66.4 / 63.1 &             88.1 \\
\rexvlml &    500{,}000 &      80.2 / \textbf{95.8} &      66.4 / 87.0 &    67.4 / \textbf{88.3} &    50.1 / 77.0 &        \textbf{73.3} &      \textbf{68.4} / \textbf{63.5} &             \textbf{88.3} \\
\bottomrule
\end{tabular}


==> tables/2023-04-03_best_overall_test+stanford.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{ll|cccccc|ccc}
\toprule
{} &             {} &          \multicolumn{2}{c}{\textbf{Flickr30k}}  &     \multicolumn{2}{c}{\textbf{MS-COCO}} &     \multicolumn{2}{c|}{\textbf{Stanford Paragraph}} &           \textbf{VALSE}  &    \textbf{VSR}  &           \textbf{SVO-Probes} \\
\textbf{Model} &          \textbf{Checkpoint}  &       TR@1/5  &          IR@1/5  &        TR@1/5 &         IR@1/5 &  TR@1/5 &         IR@1/5 &             Acc$_\text{r}$ &    Dev / Test Acc &                     Acc$_\text{r}$ \\
\midrule
\gray{CLIP$_\text{400M}$} & & \gray{88.0 / ?} & \gray{68.7 / ?} & \gray{58.4 / ?} & \gray{37.8 / ?} & \gray{? / ?} & \gray{? / ?} & \gray{64.0} & \gray{? / ?} & \gray{81.6} \\
\midrule
\albefb &       200{,}000 &      77.9 / 92.7 &      61.3 / 83.6 &    63.6 / 86.1 &    47.4 / 74.5 &     79.5 / 95.6 &     79.8 / 94.9 &        69.4 &      63.7 / 60.1 &             86.6 \\
\realbefb &       350000 &      76.5 / 93.0 &      61.7 / 84.0 &    63.9 / 86.7 &    47.3 / 74.8 &     85.7 / 97.6 &     85.8 / 97.3 &        70.8 &      65.5 / 60.2 &             86.7 \\
\xvlmb &       100000 &      80.4 / 94.8 &      63.7 / 86.4 &    66.4 / 87.8 &    49.1 / 76.3 &     80.4 / 94.9 &     80.2 / 95.0 &        68.5 &      64.0 / 61.7 &             87.0 \\
\rexvlmb &       250000 &      77.6 / 94.4 &      61.8 / 84.3 &    66.8 / 88.2 &    49.4 / 76.2 &     87.1 / 98.0 &     88.3 / 97.4 &        71.2 &      66.6 / 62.6 &             87.2 \\
\midrule
\albefl &       250000 &      84.1 / 94.6 &      67.3 / 87.6 &    66.8 / 87.9 &    49.7 / 76.5 &     82.3 / 96.1 &     82.6 / 95.8 &        71.4 &      62.4 / 61.3 &             87.5 \\
\realbefl &       500000 &      80.3 / 93.7 &      65.1 / 86.0 &    66.3 / 87.8 &    49.1 / 76.1 &     87.0 / 97.3 &     86.5 / 97.3 &        70.4 &      64.6 / 61.3 &             87.7 \\
\xvlml &       150000 &      83.5 / 95.5 &      67.5 / 88.6 &    67.6 / 87.9 &    50.6 / 77.1 &     84.4 / 96.5 &     84.6 / 96.6 &        70.9 &      66.4 / 63.1 &             88.3 \\
\rexvlml &       500000 &      80.2 / 95.8 &      66.4 / 87.0 &    67.4 / 88.3 &    50.1 / 77.0 &     89.7 / 98.0 &     88.7 / 97.9 &        73.3 &      68.4 / 63.5 &             88.1 \\
\bottomrule
\end{tabular}

==> tables/2023-04-17_fixed_test.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{l|ccccc|cccc}
\toprule
{} &     \multicolumn{2}{c}{\textbf{Stanford Paragraph}} &           \textbf{VALSE}  &    \textbf{VSR Random}  &           \multicolumn{1}{c|}{\textbf{SVO}} &          \multicolumn{2}{c}{\textbf{Flickr30K}}  &     \multicolumn{2}{c}{\textbf{COCO}} \\
\textbf{Model} &       TR@1/5 &         IR@1/5 &             Acc$_\text{r}$ &    Dev / Test Acc &                     Acc$_\text{r}$ & TR@1/5  &          IR@1/5  &        TR@1/5 &         IR@1/5 \\
\midrule
\gray{CLIP$_\text{400M}$} & \gray{? / ?} & \gray{? / ?} & \gray{64.0} & \gray{N/A} & \gray{81.6} & \gray{88.0 / ?} & \gray{68.7 / ?} & \gray{58.4 / ?} & \gray{37.8 / ?} \\
\midrule
\albefb   &     79.5 / 95.6 &     79.8 / 94.9 &        69.4 &      63.7 / 60.1 &             86.6 & 77.9 / 92.7 &      61.3 / 83.6 &    63.6 / 86.1 &    47.4 / 74.5 \\
\realbefb &     85.1 / 97.4 &     85.8 / 97.2 &        69.6 &      64.1 / 60.1 &             86.2 & 75.5 / 92.3 &      59.5 / 82.6 &    62.7 / 86.2 &    46.4 / 74.7 \\
\xvlmb    &     79.8 / 94.8 &     81.4 / 95.0 &        69.5 &      63.4 / \textbf{62.4} &             \textbf{87.3} & 78.2 / \textbf{94.1} &      \textbf{61.8} / 84.1 &    63.9 / 86.7 &    47.9 / 74.7 \\
\rexvlmb  &     \textbf{87.4} / \textbf{97.8} &     \textbf{87.8} / \textbf{97.4} &        \textbf{70.9} &      \textbf{64.9} / 61.8 &             87.2 & \textbf{78.6} / 93.9 &      \textbf{61.8} / \textbf{84.8} &    \textbf{66.0} / \textbf{87.5} &    \textbf{48.9} / \textbf{76.2}  \\
\midrule
\albefl   &     75.4 / 93.1 &     71.7 / 89.2 &        72.2 &      60.4 / 59.4 &             86.7 & \textbf{82.2} / 95.5 &      66.1 / 85.8 &    64.8 / 86.6 &    49.1 / 74.6 \\
\realbefl &     87.0 / 97.3 &     86.5 / 97.3 &        70.4 &      64.6 / 61.3 &             87.7 & 80.3 / 93.7 &      65.1 / 86.0 &    66.3 / 87.8 &    49.1 / 76.1 \\
\xvlml    &     79.3 / 94.7 &     76.6 / 92.0 &        71.3 &      61.1 / 60.5 &             87.3 & 82.1 / 94.9 &      65.0 / 85.9 &    64.7 / 86.5 &    49.0 / 74.6 \\
\rexvlml  &     \textbf{89.7} / \textbf{98.0} &     \textbf{88.7} / \textbf{97.9} &        \textbf{73.3} &      \textbf{68.4} / \textbf{63.5} &             \textbf{88.3} & 80.2 / \textbf{95.8} &      \textbf{66.4} / \textbf{87.0} &    \textbf{67.4} / \textbf{88.3} &    \textbf{50.1} / \textbf{77.0} \\
\bottomrule
\end{tabular}

% 0  &                   albef-500k@200k &     79.5 / 95.6 &     79.8 / 94.9 &        69.4 &      63.7 / 60.1 &             86.6 &      77.9 / 92.7 &      61.3 / 83.6 &    63.6 / 86.1 &    47.4 / 74.5 \\
% 6  &  albef-mix-models-relclf-vsg@200k &     85.1 / 97.4 &     85.8 / 97.2 &        69.6 &      64.1 / 60.1 &             86.2 &      75.5 / 92.3 &      59.5 / 82.6 &    62.7 / 86.2 &    46.4 / 74.7 \\
% 8  &                    xvlm-500k@200k &     79.8 / 94.8 &     81.4 / 95.0 &        69.5 &      63.4 / 62.4 &             87.3 &      78.2 / 94.1 &      61.8 / 84.1 &    63.9 / 86.7 &    47.9 / 74.7 \\
% 14 &   xvlm-mix-models-relclf-vsg@200k &     87.4 / 97.8 &     87.8 / 97.4 &        70.9 &      64.9 / 61.8 &             87.2 &      78.6 / 93.9 &      61.8 / 84.8 &    66.0 / 87.5 &    48.9 / 76.2 \\

% 0  &                        albef-14m@500k &     75.4 / 93.1 &     71.7 / 89.2 &        72.2 &      60.4 / 59.4 &             86.7 &      82.2 / 95.5 &      66.1 / 85.8 &    64.8 / 86.6 &    49.1 / 74.6 \\
% 6  &  albef-mix-models-relclf-vsg-14m@500k &     87.0 / 97.3 &     86.5 / 97.3 &        70.4 &      64.6 / 61.3 &             87.5 &      80.3 / 93.7 &      65.1 / 86.0 &    66.3 / 87.8 &    49.1 / 76.1 \\
% 8  &                    xvlm-500k-14m@500k &     79.3 / 94.7 &     76.6 / 92.0 &        71.3 &      61.1 / 60.5 &             87.3 &      82.1 / 94.9 &      65.0 / 85.9 &    64.7 / 86.5 &    49.0 / 74.6 \\
% 13 &   xvlm-mix-models-relclf-vsg-14m@500k &     89.7 / 98.0 &     88.7 / 97.9 &        73.3 &      68.4 / 63.5 &             88.1 &      80.2 / 95.8 &      66.4 / 87.0 &    67.4 / 88.3 &    50.1 / 77.0 \\

==> tables/2023-05-07_coco_test.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{l|ccccc|cccc}
\toprule
{} &     \multicolumn{2}{c}{\textbf{Stanford Paragraph}} &           \textbf{VALSE}  &    \textbf{VSR Random}  &           \multicolumn{1}{c|}{\textbf{SVO}} &          \multicolumn{2}{c}{\textbf{Flickr30K}}  &     \multicolumn{2}{c}{\textbf{COCO}} \\
\textbf{Model} &       TR@1/5 &         IR@1/5 &             Acc$_\text{r}$ &    Dev / Test Acc &                     Acc$_\text{r}$ & TR@1/5  &          IR@1/5  &        TR@1/5 &         IR@1/5 \\
\midrule
\gray{CLIP$_\text{400M}$} & \gray{? / ?} & \gray{? / ?} & \gray{64.0} & \gray{N/A} & \gray{81.6} & \gray{88.0 / ?} & \gray{68.7 / ?} & \gray{58.4 / ?} & \gray{37.8 / ?} \\
\midrule
\albefb   &     77.9 / 94.5 &     79.8 / 94.7 &        68.9 &      61.4 / 60.3 &             \textbf{87.4} &      78.4 / 93.5 &      61.2 / 84.6 &    63.9 / 86.5 &    47.4 / 74.9 \\
\realbefb &     85.7 / 97.6 &     85.8 / 97.3 &        70.8 &      65.5 / 60.2 &             86.7 &      76.5 / 93.0 &      61.7 / 84.0 &    63.9 / 86.7 &    47.3 / 74.8 \\
\xvlmb    &     80.4 / 94.9 &     80.2 / 95.0 &        68.5 &      64.0 / 61.7 &             87.0 &      \textbf{80.4} / \textbf{94.8} &      \textbf{63.7} / \textbf{86.4} &    66.4 / 87.8 &    49.1 / \textbf{76.3} \\
\rexvlmb  &     \textbf{87.1} / \textbf{98.0} &     \textbf{88.3} / \textbf{97.4} &        \textbf{71.2} &      \textbf{66.6} / \textbf{62.6} &             87.2 &      77.6 / 94.4 &      61.8 / 84.3 &    \textbf{66.8} / \textbf{88.2} &    \textbf{49.4} / 76.2 \\
\midrule
\albefl   &     82.3 / 96.1 &     82.6 / 95.8 &        71.4 &      62.4 / 61.3 &             87.7 &      84.1 / 94.6 &      67.3 / 87.6 &    66.8 / 87.9 &    49.7 / 76.5 \\
\realbefl &     84.7 / 96.8 &     85.4 / 96.3 &        72.2 &      64.5 / 62.5 &             87.7 &      \textbf{84.2} / \textbf{96.6} &      \textbf{68.0} / \textbf{87.8} &    67.3 / 88.4 &   \textbf{50.7} / 76.9 \\
\xvlml    &     79.3 / 94.7 &     76.6 / 92.0 &        71.3 &      61.1 / 60.5 &             87.3 & 82.1 / 94.9 &      65.0 / 85.9 &    64.7 / 86.5 &    49.0 / 74.6 \\
\rexvlml  &     \textbf{89.9} / \textbf{97.8} &     \textbf{88.7} / \textbf{98.0} &        \textbf{73.5} &      \textbf{68.1} / \textbf{62.4} &             \textbf{88.0} &      81.1 / 94.8 &      65.7 / 87.3 &    \textbf{67.4} / \textbf{89.0} &    50.3 / \textbf{77.3} \\
\bottomrule
\end{tabular}



==> tables/2023-05-12_coco_test.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{l|ccc|cccc}
\toprule
{} &     \textbf{VALSE}  &    \textbf{VSR Random}  &           \multicolumn{1}{c|}{\textbf{SVO-Probes}} &          \multicolumn{2}{c}{\textbf{Flickr30K}}  &     \multicolumn{2}{c}{\textbf{COCO}} \\
\textbf{Model} &       Acc$_\text{r}$ &    Dev / Test Acc &                     Acc$_\text{r}$ & TR@1/5  &          IR@1/5  &        TR@1/5 &         IR@1/5 \\
\midrule
\gray{CLIP$_\text{400M}$} & \gray{64.0} & \gray{N/A} & \gray{81.6} & \gray{88.0 / 98.7} & \gray{68.7 / 90.6} & \gray{58.4 / 81.5} & \gray{37.8 / 62.4} \\
\gray{BLIP-2$_\text{129M}$} & \gray{74.0} & \gray{61.2 / 61.5} & \gray{86.5} & \gray{95.5 / 99.9} & \gray{86.7 / 97.1} & \gray{80.7 / 94.7} & \gray{64.2 / 85.2} \\
\midrule
\albefb   &     68.9 &      61.4 / 60.3 &             \textbf{87.4} &      78.4 / 93.5 &      61.2 / 84.6 &    63.9 / 86.5 &    47.4 / 74.9 \\
\realbefb &     \better{70.8} &      \better{65.5} / \worse{60.2} &             \worse{86.7} &      \worse{76.5} / \worse{93.0} &      \better{61.7} / \worse{84.0} &    63.9 / \better{86.7} &    \worse{47.3} / \worse{74.8} \\
\xvlmb    &     68.5 &      64.0 / 61.7 &             87.0 &      \textbf{80.4} / \textbf{94.8} &      \textbf{63.7} / \textbf{86.4} &    66.4 / 87.8 &    49.1 / \textbf{76.3} \\
\rexvlmb  &     \textbf{\better{71.2}} &      \textbf{\better{66.6}} / \textbf{\better{62.6}} &             \better{87.2} &      \worse{77.6} / \worse{94.4} &      \worse{61.8} / \worse{84.3} &    \textbf{\better{66.8}} / \textbf{\better{88.2}} &    \textbf{\better{49.4}} / \worse{76.2} \\
\midrule
\albefl   &     71.4 &      62.4 / 61.3 &             87.7 &      84.1 / 94.6 &      67.3 / 87.6 &    66.8 / 87.8 &    49.7 / 76.5 \\
\realbefl &     \worse{71.1} &      \better{63.5} / {\better{61.5}} &             87.7 &      {\worse{80.3}} / {\worse{93.6}} &      {\worse{64.9}} / {\worse{85.6}} &    \worse{66.5} / {87.8} &   {\worse{48.8}} / \worse{75.9} \\
\xvlml    &     72.2 &      64.5 / \textbf{62.5} &             87.7 & \textbf{84.2} / \textbf{96.6} &      \textbf{68.0} / \textbf{87.8} &    67.3 / 88.4 &    \textbf{50.7} / 76.9 \\
\rexvlml  &     \textbf{\better{73.5}} &      \textbf{\better{68.1}} / {\textbf{62.5}} &             \textbf{\better{88.0}} &      \worse{81.1} / \worse{94.8} &      \worse{65.7} / \worse{87.3} &    \textbf{\better{67.4}} / \textbf{\better{89.0}} &    \worse{50.3} / \textbf{\better{77.3}} \\
\bottomrule
\end{tabular}


==> tables/2023-05-12_fixed_test.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{l|ccc|cccc}
\toprule
{} &     \textbf{VALSE}  &    \textbf{VSR Random}  &           \multicolumn{1}{c|}{\textbf{SVO-Probes}} &          \multicolumn{2}{c}{\textbf{Flickr30K}}  &     \multicolumn{2}{c}{\textbf{COCO}} \\
\textbf{Model} &       Acc$_\text{r}$ &    Dev / Test Acc &                     Acc$_\text{r}$ & TR@1/5  &          IR@1/5  &        TR@1/5 &         IR@1/5 \\
\midrule
% \gray{CLIP$_\text{400M}$} & \gray{64.0} & \gray{N/A} & \gray{81.6} & \gray{88.0 / ?} & \gray{68.7 / ?} & \gray{58.4 / ?} & \gray{37.8 / ?} \\
% \midrule
\albefb   &     69.4 &      63.7 / 60.1 &             86.6 & 77.9 / 92.7 &      61.3 / 83.6 &    63.6 / 86.1 &    47.4 / 74.5 \\
\realbefb &     \better{69.6} &      \better{64.0} / \better{60.2} &             \worse{86.2} & \worse{75.5} / \worse{92.3} &      \worse{59.5} / \worse{82.6} &    \worse{62.7} / \better{86.2} &    \worse{46.4} / \better{74.7} \\
\xvlmb    &     69.5 &      63.4 / \textbf{62.4} &             \textbf{87.3} & 78.2 / \textbf{94.1} &      \textbf{61.8} / 84.1 &    63.9 / 86.7 &    47.9 / 74.7 \\
\rexvlmb  &     \textbf{\better{70.9}} &      \textbf{\better{65.0}} / \worse{61.8} &             \worse{87.2} & \textbf{\better{78.6}} / \worse{93.9} &      \textbf{61.8} / \textbf{\better{84.8}} &    \textbf{\better{66.0}} / \textbf{\better{87.5}} &    \textbf{\better{48.9}} / \textbf{\better{76.2}}  \\
\midrule
\albefl   &     72.2 &      60.4 / 59.4 &             86.7 & \textbf{82.2} / 95.5 &      66.1 / 85.8 &    64.8 / 86.6 &    49.1 / 74.6 \\
\realbefl &     \worse{70.4} &      \better{64.6} / \better{61.3} &             \better{87.7} & \worse{80.3} / \worse{93.7} &      \worse{65.1} / \better{86.0} &    \better{66.3} / \better{87.8} &    49.1 / \better{76.1} \\
\xvlml    &     71.3 &      61.1 / 60.5 &             87.3 & 82.1 / 94.9 &      65.0 / 85.9 &    64.7 / 86.5 &    49.0 / 74.6 \\
\rexvlml  &     \textbf{\better{73.3}} &      \textbf{\better{68.4}} / \textbf{\better{63.5}} &             \textbf{\better{88.3}} & \worse{80.2} / \textbf{\better{95.8}} &      \textbf{\better{66.4}} / \textbf{\better{87.0}} &    \textbf{\better{67.4}} / \textbf{\better{88.3}} &    \textbf{\better{50.1}} / \textbf{\better{77.0}} \\
\bottomrule
\end{tabular}

% 0  &                   albef-500k@200k &     79.5 / 95.6 &     79.8 / 94.9 &        69.4 &      63.7 / 60.1 &             86.6 &      77.9 / 92.7 &      61.3 / 83.6 &    63.6 / 86.1 &    47.4 / 74.5 \\
% 6  &  albef-mix-models-relclf-vsg@200k &     85.1 / 97.4 &     85.8 / 97.2 &        69.6 &      64.1 / 60.1 &             86.2 &      75.5 / 92.3 &      59.5 / 82.6 &    62.7 / 86.2 &    46.4 / 74.7 \\
% 8  &                    xvlm-500k@200k &     79.8 / 94.8 &     81.4 / 95.0 &        69.5 &      63.4 / 62.4 &             87.3 &      78.2 / 94.1 &      61.8 / 84.1 &    63.9 / 86.7 &    47.9 / 74.7 \\
% 14 &   xvlm-mix-models-relclf-vsg@200k &     87.4 / 97.8 &     87.8 / 97.4 &        70.9 &      64.9 / 61.8 &             87.2 &      78.6 / 93.9 &      61.8 / 84.8 &    66.0 / 87.5 &    48.9 / 76.2 \\

% 0  &                        albef-14m@500k &     75.4 / 93.1 &     71.7 / 89.2 &        72.2 &      60.4 / 59.4 &             86.7 &      82.2 / 95.5 &      66.1 / 85.8 &    64.8 / 86.6 &    49.1 / 74.6 \\
% 6  &  albef-mix-models-relclf-vsg-14m@500k &     87.0 / 97.3 &     86.5 / 97.3 &        70.4 &      64.6 / 61.3 &             87.5 &      80.3 / 93.7 &      65.1 / 86.0 &    66.3 / 87.8 &    49.1 / 76.1 \\
% 8  &                    xvlm-500k-14m@500k &     79.3 / 94.7 &     76.6 / 92.0 &        71.3 &      61.1 / 60.5 &             87.3 &      82.1 / 94.9 &      65.0 / 85.9 &    64.7 / 86.5 &    49.0 / 74.6 \\
% 13 &   xvlm-mix-models-relclf-vsg-14m@500k &     89.7 / 98.0 &     88.7 / 97.9 &        73.3 &      68.4 / 63.5 &             88.1 &      80.2 / 95.8 &      66.4 / 87.0 &    67.4 / 88.3 &    50.1 / 77.0 \\

==> tables/2023-05-18_auc_test.tex <==
\definecolor{LightCyan}{rgb}{0.94,0.94,0.94}

\hypersetup{citecolor=lightgray}
\begin{tabular}{l|ccc|cccc}
\toprule
{} &     \textbf{VALSE}  &    \textbf{VSR Random}  &           \multicolumn{1}{c|}{\textbf{SVO-Probes}} &          \multicolumn{2}{c}{\textbf{Flickr30K}}  &     \multicolumn{2}{c}{\textbf{COCO}} \\
\textbf{Model} &       Acc$_\text{r}$ &    Dev / Test Acc &                     Acc$_\text{r}$ & TR@1/5  &          IR@1/5  &        TR@1/5 &         IR@1/5 \\
\midrule
\rowcolor{LightCyan} \albefb   &     55.1 &  49.7 / 48.0 & 69.3 & 61.9 / 74.4 & 48.8 / 66.8 & 50.0 / 68.3 & 37.5 / 59.2 \\
\rowcolor{LightCyan} \realbefb &     \better{56.1} & \better{51.1} / \worse{47.6} & \worse{68.8} & \worse{59.3} / \worse{73.3} & \worse{46.9} / \worse{65.8} & \worse{49.1} / 68.3 & \worse{36.5} / 59.2 \\
\rowcolor{LightCyan} \xvlmb    &     55.7 & 50.3 / 48.7 & \textbf{69.6} & \textbf{63.1} / \textbf{75.3} & \textbf{49.5} / \textbf{67.4} & 51.2 / 68.9 & 38.3 / 59.4 \\
\rowcolor{LightCyan} \rexvlmb  &     \textbf{\better{56.5}} & \textbf{\better{52.1}} / \textbf{\better{49.5}} & \textbf{69.6} & \worse{62.0} / \worse{74.7} & \worse{48.6} / 67.4 & \textbf{\better{51.7}} / \textbf{\better{69.7}} & \textbf{\better{38.5}} / \textbf{\better{60.5}} \\
\midrule
\rowcolor{LightCyan} \albefl   & 57.1 & 49.8 / 48.6 & 70.0 & 65.9 / 75.9 & 52.7 / 69.7 & 52.5 / 69.9 & 39.3 / 60.8 \\
\rowcolor{LightCyan} \realbefl & \worse{56.6} & \better{50.0} / \worse{48.1} & \worse{69.5} & \worse{61.3} / \worse{74.2} & \worse{49.2} / \worse{67.5} & \worse{50.1} / \worse{68.8} & \worse{37.2} / \worse{59.7} \\
\rowcolor{LightCyan} \xvlml    & 57.3 & 50.8 / 49.2 & \textbf{70.2} & \textbf{66.5} / \textbf{76.8} & \textbf{53.7} / \textbf{70.1} & \textbf{53.3} / \textbf{70.3} & \textbf{40.2} / \textbf{61.2} \\
\rowcolor{LightCyan} \rexvlml  & \textbf{\better{57.4}} & \textbf{\better{52.6}} / \textbf{\better{49.4}} & \textbf{70.2} & \worse{63.1} / \worse{75.4} & \worse{50.9} / \worse{69.0} & \worse{52.2} / \textbf{70.3} & \worse{39.0} / \textbf{61.2} \\
\bottomrule
\end{tabular}

==> tables/2023-05-23_coco_test.tex <==
albef-500k & 68.9 & 61.4 & 60.3 & 87.4 & 78.4 & 61.2 & 63.9 & 47.4 & \\
albef-mix-models-relclf-vsg & 70.8 & 65.5 & 60.2 & 86.7 & 76.5 & 61.7 & 63.9 & 47.3 & \\
xvlm-500k & 68.5 & 64.0 & 61.7 & 87.0 & 80.4 & 63.7 & 66.4 & 49.1 & \\
xvlm-mix-models-relclf-vsg & 71.2 & 66.6 & 62.6 & 87.2 & 77.6 & 61.8 & 66.8 & 49.4 & \\

albef-14m & 71.4 & 62.4 & 61.3 & 87.7 & 84.1 & 67.3 & 66.8 & 49.7 & \\
albef-mix-models-relclf-vsg-14m & 71.1 & 63.5 & 61.5 & 87.6 & 80.3 & 64.9 & 66.5 & 48.8 & \\
xvlm-500k-14m & 72.2 & 64.5 & 62.5 & 87.7 & 84.2 & 68.0 & 67.3 & 50.7 & \\
xvlm-mix-models-relclf-vsg-14m & 73.5 & 68.1 & 62.4 & 88.0 & 81.1 & 65.7 & 67.4 & 50.3 & \\

==> tables/2023-06-15_cg-test_fixed.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{l|ccccc}
\toprule
{} &     \multicolumn{2}{c}{\textbf{Flickr30K}} & \multicolumn{2}{c}{\textbf{COCO}} \\
\textbf{Model} &  IR@1/5  &        TR@1/5 & IR@1/5  &        TR@1/5 \\
\midrule
\gray{CLIP$_\text{400M}$} & \gray{88.0 / 98.7} & \gray{68.7 / 90.6} & \gray{58.4 / 81.5} & \gray{37.8 / 62.4} \\
\gray{BLIP-2$_\text{129M}$} & \gray{95.5 / 99.9} & \gray{86.7 / 97.1} & \gray{80.7 / 94.7} & \gray{64.2 / 85.2} \\
\midrule
\albefb   & 77.9 / 92.7 &      61.3 / 83.6 &    63.6 / 86.1 &    47.4 / 74.5 \\
\realbefb & \worse{75.5} / \worse{92.3} &      \worse{59.5} / \worse{82.6} &    \worse{62.7} / \better{86.2} &    \worse{46.4} / \better{74.7} \\
\xvlmb    & 78.2 / \textbf{94.1} &      \textbf{61.8} / 84.1 &    63.9 / 86.7 &    47.9 / 74.7 \\
\rexvlmb  & \textbf{\better{78.6}} / \worse{93.9} &      \textbf{61.8} / \textbf{\better{84.8}} &    \textbf{\better{66.0}} / \textbf{\better{87.5}} &    \textbf{\better{48.9}} / \textbf{\better{76.2}}  \\
\midrule
\albefl   &     \textbf{82.2} / 95.5 &      66.1 / 85.8 &    64.8 / 86.6 &    49.1 / 74.6 \\
\realbefl &     \worse{80.3} / \worse{93.7} &      \worse{65.3} / \better{86.0} &    \better{66.4} / \better{87.8} &    49.1 / \better{76.1} \\
\xvlml    &     83.3 / 95.6 &      66.2 / 86.3 &    64.1 / 86.4 &    49.1 / 74.8 \\
\rexvlml  &     \worse{80.3} / \textbf{\better{95.8}} &      \textbf{\better{66.6}} / \textbf{\better{87.0}} &    \textbf{\better{66.9}} / \textbf{\better{88.9}} &    \textbf{\better{50.2}} / \textbf{\better{77.0}} \\
\bottomrule
\end{tabular}


==> tables/2023-06-15_fg-test_fixed.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{l|ccccc}
\toprule
{} & \textbf{VSR Random}  &           \textbf{VALSE}  &    \multicolumn{1}{c}{\textbf{SVO-Probes}} & \multicolumn{2}{c}{\textbf{Stanford Paragraphs}} \\
\textbf{Model} &    Dev / Test Acc &      Acc$_\text{r}$ &    Acc$_\text{r}$ &  IR@1/5  &        TR@1/5 \\
\midrule
\gray{CLIP$_\text{400M}$}  & \gray{N/A$^\dagger$}  & \gray{64.0} & \gray{81.6} & \gray{45.3 / 73.1} & \gray{53.4 / 80.1} \\
\gray{BLIP-2$_\text{129M}$} & \gray{61.2 / 61.5} & \gray{74.0} &  \gray{86.5} & \gray{83.4 / 95.2} & \gray{81.1 / 94.3} \\
\midrule
\albefb   &     63.7 / 60.1 & 69.4 & 86.6 & 79.5 / 95.6 & 79.8 / 94.9 \\
\realbefb &     \better{64.0} / \better{60.2} & \better{69.6} & \worse{86.2} & \better{85.1} / \better{97.4} & \better{85.8} / \better{97.2} \\
\xvlmb    &     63.5 / \textbf{62.3} & 69.5 & \textbf{87.3} & 79.8 / 94.8 & 81.4 / 95.0 \\
\rexvlmb  &     \better{\textbf{65.0}} / \worse{61.8} & \better{\textbf{70.9}} & \textbf{87.3} & \better{\textbf{87.4}} / \better{\textbf{97.8}} & \better{\textbf{87.8}} / \better{\textbf{97.4}} \\
\midrule
\albefl   &     61.4 / 60.4 & 72.6 & 87.2 & 77.1 / 93.7 & 73.7 / 90.3 \\
\realbefl &     \better{65.2} / \better{61.2} & \worse{71.0} & \better{87.6} & \better{86.7} / \better{97.5} & \better{86.5} / \better{97.2} \\
\xvlml    &     61.4 / 59.7 & 71.4 & 87.4 & 80.3 / 94.9 & 76.8 / 92.4 \\
\rexvlml  &     \better{\textbf{68.2}} / \better{\textbf{62.7}} & \better{\textbf{73.1}} & \better{\textbf{88.2}} & \better{\textbf{89.3}} / \better{\textbf{98.0}} & \better{\textbf{88.8}} / \better{\textbf{97.7}}\\
\bottomrule
\end{tabular}


==> tables/2023-06-19_fg-test_fixed.tex <==
\hypersetup{citecolor=lightgray}
\begin{tabular}{l|ccccc}
\toprule
{} & \textbf{VSR Random}  &           \textbf{VALSE}  &    \multicolumn{1}{c}{\textbf{SVO-Probes}} & \multicolumn{2}{c}{\textbf{Stanford Paragraphs}} \\
\textbf{Model} &    Dev / Test Acc &      Acc$_\text{r}$ &    Acc$_\text{r}$ &  IR@1/5  &        TR@1/5 \\
\midrule
\gray{CLIP$_\text{400M}$}  & \gray{N/A$^\dagger$}  & \gray{64.0} & \gray{81.6} & \gray{45.3 / 73.1} & \gray{53.4 / 80.1} \\
\gray{BLIP-2$_\text{129M}$} & \gray{61.2 / 61.5} & \gray{74.0} &  \gray{86.5} & \gray{83.4 / 95.2} & \gray{81.1 / 94.3} \\
\midrule
\albefb   &     63.7 / 60.1 & 69.4 & 86.6 & 79.5 / 95.6 & 79.8 / 94.9 \\
\realbefb &     \ulbetter{64.0} / \ulbetter{60.2} & \ulbetter{69.6} & \ulworse{86.2} & \ulbetter{85.1} / \ulbetter{97.4} & \ulbetter{85.8} / \ulbetter{97.2} \\
\xvlmb    &     63.5 / \textbf{62.3} & 69.5 & \textbf{87.3} & 79.8 / 94.8 & 81.4 / 95.0 \\
\rexvlmb  &     \ulbetter{\textbf{65.0}} / \ulworse{61.8} & \ulbetter{\textbf{70.9}} & \textbf{87.3} & \ulbetter{\textbf{87.4}} / \ulbetter{\textbf{97.8}} & \ulbetter{\textbf{87.8}} / \ulbetter{\textbf{97.4}} \\
\midrule
\albefl   &     61.4 / 60.4 & 72.6 & 87.2 & 77.1 / 93.7 & 73.7 / 90.3 \\
\realbefl &     \ulbetter{65.2} / \ulbetter{61.2} & \ulworse{71.0} & \ulbetter{87.6} & \ulbetter{86.7} / \ulbetter{97.5} & \ulbetter{86.5} / \ulbetter{97.2} \\
\xvlml    &     61.4 / 59.7 & 71.4 & 87.4 & 80.3 / 94.9 & 76.8 / 92.4 \\
\rexvlml  &     \ulbetter{\textbf{68.2}} / \ulbetter{\textbf{62.7}} & \ulbetter{\textbf{73.1}} & \ulbetter{\textbf{88.2}} & \ulbetter{\textbf{89.3}} / \ulbetter{\textbf{98.0}} & \ulbetter{\textbf{88.8}} / \ulbetter{\textbf{97.7}}\\
\bottomrule
\end{tabular}


==> tables/benchmarks.tex <==
% \definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{LightCyan}{rgb}{0.96,0.96,0.96}

\hypersetup{citecolor=lightgray}
\begin{tabular}{l l rc l}
\toprule
\textbf{Benchmark} & \textbf{Task} & \textbf{Examples} & \textbf{Subtasks} & \textbf{Example Subtasks}  \\
\midrule
 \multicolumn{5}{c}{\emph{Fine-grained Tasks}} \\
 \midrule
 \rowcolor{LightCyan}
SVO-Probes  & Verb            & 48K & 3 & subject, verb, object \\
\rowcolor{LightCyan}
 & understanding            &  &  &  \\
VALSE       & \vl                 & 14K & 6 & existence, counting,  \\
 & grounding            &  &  &  spatial relations\\
 \rowcolor{LightCyan}
VSR         & Spatial             & (1K) 2K  & 7 & adjacency, directional, \\
\rowcolor{LightCyan}
 & reasoning           &  &  &  proximity relationships\\
Winoground  & Compositional      & 800 & 8 & pragmatics, object swap, \\
 & reasoning           &  &  &  relation swap\\
\midrule
\multicolumn{5}{c}{\emph{Coarse-grained Tasks}} \\
\midrule
\rowcolor{LightCyan}
COCO & Retrieval &  (25K) 25K & 0  & N/A\\
Flickr30K & Retrieval &  (5K) 5K & 0 & N/A \\
\bottomrule
\end{tabular}
